Defects and Frustration in the Packing of Soft Balls

This work introduces the Hookean-Voronoi energy, a minimal model for the packing of soft, deformable balls. This is motivated by recent studies of quasi-periodic equilibria arising from dense packings of diblock and star polymers. Restricting to the planar case, we investigate the equilibrium packings of identical, deformable objects whose shapes are determined by an $N$-site Voronoi tessellation of a periodic rectangle. We derive a reduced formulation of the system showing at equilibria each site must reside at the ``max-center'' of its associated Voronoi region and construct a family of ordered ``single-string'' minimizers whose cardinality is $O(N^2)$. We identify sharp conditions under which the system admits a regular hexagonal tessellation and establish that in all cases the average energy per site is bounded below by that of a regular hexagon of unit size. However, numerical investigation of gradient flow of random initial data, reveals that for modest values of $N$ the system preponderantly equilibrates to quasi-ordered states with low energy and large basins of attraction. For larger $N$ the distribution of equilibria energies appears to approach a $\delta$-function limit, whose energy is significantly higher than the ground state hexagon. This limit is possibly shaped by two mechanisms: a proliferation of moderate-energy disordered equilibria that block access of the gradient flow to lower energy quasi-ordered states and a rigid threshold on the maximum energy of stable states.

==> Cut-material.tex <==
\subsection*{Low defect penta-hepta Tessellations}
Let $\bx$ be a collection of $N$ sites, whose Voronoi tessellation of $\Omega_\alpha$ is formed by $\{\region{i}\}_{i=1}^N$. Assume the tessellation has $D$ pairs of penta-hepta defects with $D/N\ll1.$ From Kenny's Lemma the $s$-sided regions $\region{i}$ enjoy the bound
$$ \bar{r}(V_i) \leq \bar{r}_s |\region{i}|^{\frac12},$$
where $\bar{r}_s$ is the average radius of the regular $s$-gon with unit area. These are increasing functions of $s$ that converge to the limit $2\pi^{\frac12}$.
Let $\Omega_s$ denote the total area occupied by $s$-sided regions, so that $|\Omega_5|+|\Omega_6|+|\Omega_7|=N.$ 
Enumerating the regions with increasing side-count the per-site average radius of the tessellation satisfies 
$$\bar{r}(\bx) :=\frac{1}{N}\sum_{i=1}^N \bar{r}(\region{i}) \leq 
\frac{1}{N}\left(\bar{r}_{5}\sum_{i=1}^D|\region{i}|^{\frac12}+
\bar{r}_{6}\sum_{i=D+1}^{N-D}|\region{i}|^{\frac12} +
\bar{r}_{7}\sum_{i=N-D+1}^{N}|\region{i}|^{\frac12}\right).
$$
Applying Holder's inequality to each of the three terms we have the estimate
$$ \bar{r}(\bx)\leq \frac{1}{N}\left( \sqrt{N-2D}|\Omega_6|^{\frac12}\bar{r}_6+
 \sqrt{D} |\Omega_5|^{\frac12}\bar{r}_5+\sqrt{D}|\Omega_7|^{\frac12}\bar{r}_7 \right),$$
 To simplify notation we introduce $\rho_{s}$ as the average area of the $s$-gons, $|\Omega_s|=\rho_s D,$ with $\rho_5<1<\rho_7$.  This affords the bound
 \beq\label{e:VEE-pos} 
 \bar{r}(\bx)\leq  \sqrt{1-2p}\sqrt{1-(\rho_5+\rho_7)p}\, \bar{r}_6+
 p(\bar{r}_5 \sqrt{\rho_5}+\bar{r}_7\sqrt{\rho_7}),
 \eeq
 where $p:=D/N\ll1$ is the ratio of defect pairs to sites. 
 
 If $p=0$, then there are no defects and we have $\bar{r}(\bx)\leq \bar{r}_6$ which implies that $\VEE(\bx)\geq0.$ For small $p$ we have the expansion
 $$ \bar{r}(\bx) \leq \bar{r}_6\left( 1 -\left( 1+\frac{\rho_5+\rho_7}{2} -\sqrt{\rho_5}\frac{\bar{r}_5}{\bar{r}_6}-\sqrt{\rho_7}\frac{\bar{r}_7}{\bar{r}_6}\right)p \right) +O(p^2). $$
 Thus if $\rho_{5}$ and $\rho_7$  satisfy
 \beq
 \label{e:VEE-pos-smallp}
 \frac{\bar{r}_5}{\bar{r}_6} \sqrt{\rho_5}+\frac{\bar{r}_7}{\bar{r}_6} \sqrt{\rho_7}<  
 1+\frac{\rho_5}{2}+\frac{\rho_7}{2},
 \eeq
 then 
 $ \bar{r}(\bx)<\bar{r}_6$ and $\VEE(\bx)> 0.$ We break this into two separate inequalities. Since $\bar{r}_5<\bar{r}_6$ the inequality
 $$ \frac{\bar{r}_5}{\bar{r}_6} \sqrt{\rho_5} < \frac{1+\rho_5}{2},$$
 holds for all $\rho_5\geq0$. Conversely the inequality
  $$ \frac{\bar{r}_7}{\bar{r}_6} \sqrt{\rho_7} <\frac{1+\rho_7}{2},$$
holds unless 
$$|\rho_7-1|<2\sqrt{2\frac{\bar{r}_7-\bar{r}_6}{\bar{r}_6}}\ll1,$$ 
where the small but non-adjustable parameter arises from the rapid convergence of the average radius of an $s$-gon to its limit. Thus if $\bx$ generates a Voronoi tessellation for which the average heptagon area is sufficiently different than $1$ and the defect ratio $p$ is sufficiently small, then $\VEE(\bx)>0.$ 
\begin{Remark}
In the case $\bar{r}_5=\bar{r}_6=\bar{r}_7$ the condition \eqref{e:VEE-pos-smallp} holds with the exception of equality at $\rho_5=\rho_7=1.$ It is likely that we can treat this problem perturbatively, so that if $\bar{r}_5+\bar{r}_7<2\bar{r}_6$ then the ground state result holds uniformly in $(\rho_5,\rho_7)$, and if $\bar{r}_5+\bar{r}_7>2\bar{r}_6$ then it holds for $(\rho_5,\rho_7)$ outside a small neighborhood of $(1,1)$. 
\end{Remark}
%\pagebreak

%\bibliographystyle{alpha}\bibliography{sample}
%\printbibliography


Our intuition would suggest that of $s$-sided polygons, regular ones would maximize their average radius when area is fixed. We will demonstrate this, but we first define $\bar{\mathbf{r}}_s$, the average radius of an $s$-sided regular polygon with unit area. We can obtain an expression from , using the symmetrical properties of a regular polygon to obtain 

If the site inside a convex polygonal region is placed at a sufficient distance \textcolor{blue}{(To ensure that $0 < \theta < \pi/2$)} from each edge, we are able to decompose the region into right triangles,

We can then consider any convex polygon as a collection of right triangles with hypotenuses $h$ and angle $\theta$, subject to the constraints that they must tile back together, along with a fixed angle sum and fixed area. However, we can simplify and decouple the problem by not requiring that the triangles tile together. The maximization over this expanded set allows us to obtain a bound which is attained at $\bar{\mathbf{r}}_s$. To show this, we introduce a useful lemma.

\def\txi{\tilde{\xi}}

\begin{Lemma}
Let a collection of $K$ right triangles be defined by hypotenuses $h_i \geq 0$ and angles $\theta_i \in [0, \pi/2]$ such that $\sum_{i=1}^K \theta_i = \phi < K\pi/2$. If the total area of the triangles is fixed to $A$, the following quantity $\xi$
\beq
    \xi = \sum_{i=1}^K h_i \txi(\theta_i) 
\eeq
has a unique critical point 
\beq
    \xi_c = \sqrt{\frac{2AK}{\sin(\phi/K)\cos(\phi/K)}}\txi(\phi/K)
\eeq
if $\left[\txi^2(\theta)/\sin(2\theta)\right]'$ is \textbf{monotonic} on $[0, \pi/2]$. If the critical point value $\xi_c$ is \textbf{monotonically increasing} in $K > \lfloor2\phi/\pi\rfloor$, we have that $\xi_c$ is the maximum attainable value of $\xi$.
\end{Lemma}

\begin{proof}
To obtain a maximum for the quantity $\xi$ subject to the constraint of fixed area $A$ and fixed sum of angles $\phi$, we show the existence of a unique critical point and demonstrate the condition for the value at the boundary to be strictly less. To start, we have the quantity
\beq
    \xi = \sum_{i=1}^K h_i \txi(\theta_i), \quad \partial_{h_i} \xi =  \txi(\theta_i), \quad \partial_{\theta_i} \xi = h_i \txi'(\theta_i),
\eeq
and constraints 
\begin{gather*}
    \mathcal{A} = \frac{1}{2} \sum_{i=1}^K h_i^2 \sin\theta_i\cos\theta_i = A, \quad \partial_{h_i}\mathcal{A} = h_i\sin\theta_i\cos\theta_i, \quad \partial_{\theta_i}\mathcal{A} = \frac{1}{2}h_i^2 \cos(2\theta_i),\\
    \alpha = \sum_{i=1}^K \theta_i = \phi, \quad \partial_{h_i} \alpha = 0, \quad \partial_{\theta_i} \alpha = 1.
\end{gather*}
Then, by Lagrange multipliers the critical point must satisfy $\nabla \xi = \lambda \nabla \mathcal{A} + \mu \nabla \alpha$, for constants $\lambda, \mu$. By equating the $h_i$ partials, we can obtain
\[
    \lambda = \frac{\txi(\theta_i)}{h_i\sin\theta_i\cos\theta_i}.
\]
Equating the $\theta_i$ partials and substituting $\lambda$ we have
\[
    \begin{aligned}
    \mu &= h_i\left( \txi'(\theta_i) - \lambda \frac{1}{2} h_i \cos(2\theta_i) \right)\\
    &= h_i\left(\txi'(\theta_i) - \txi(\theta_i)\frac{\cos(2\theta_i)}{\sin(2\theta_i)} \right).
    \end{aligned}
\]
Noticing their product eliminates $h_i$,
\begin{equation}
    \begin{aligned}
    \lambda\mu = f(\theta_i) &= \frac{\txi(\theta_i)}{h_i\sin\theta_i\cos\theta_i}\left(\txi'(\theta_i) - \txi(\theta_i)\frac{\cos(2\theta_i)}{\sin(2\theta_i)} \right)\\
    &= \frac{2\sin(2\theta_i) \txi(\theta_i)\txi'(\theta_i) - 2\txi^2(\theta_i)\cos(2\theta_i)}{\sin^2(2\theta_i)} = \left(\frac{\txi^2(\theta_i)}{\sin(2\theta_i)}\right)'.
    \end{aligned}
\end{equation}
Requiring that $f$ be monotonic on $[0, \pi/2]$ implies $\theta_1 = \dots \theta_K = \phi/K$. Then, since $\mu$ is linear in $h_i$, we similarly obtain $h_1 = \dots = h_K = 2\sqrt{A/K\sin(2\phi/K)}$, the last equality obtained from the area constraint. This gives us the first condition on $\txi$. The critical point $\xi_c$ then attains the value
\beq
    \xi_c = \sqrt{\frac{2AK}{\sin(\phi/K)\cos(\phi/K)}}\txi(\phi/K)
\eeq
To ensure this is the maximum, we observe that the boundary cases where $h_i = 0$ or $\theta_i=0,\pi/2$ imply an elimination of a triangle. If we require that $\xi_c$ monotonically increases in $K$, for $K > \lfloor\phi/(\pi/2)\rfloor$, we see a maximization using fewer triangles is strictly less, and we have our result.

\end{proof}

This provides the basis for the next few results.

\begin{Theorem}
The average radius of an $s$-sided convex polygon and area $A$ has the bound
\beq
    \bar{r} \leq \bar{\mathbf{r}}_s \sqrt{A}.
\eeq
\end{Theorem}

\begin{proof}
As observed in Figure \ref{f:polygon_triangle}, we are able to decompose a regular polygon into right triangles if the center is ``well-placed". Specifically, for an convex polygon with area $A$ and $s$ sides, we can decompose it $K=2s$ triangles, and an angle sum constraint of $\sum_{i=1}^{K} \theta_i = \pi(s-2)=\phi$. From \eqref{e:barr-exact} we can write the average radius of this polygon as a sum across each triangle,
\beq\label{e:barr-triangle-decomp}
    \bar{r} = \frac{1}{2\pi} \sum_{i=1}^{K} h_i \sin\theta_i \arctanh(\cos\theta_i) = \sum_{i=1}^{K} h_i \txi(\theta_i), \quad \txi(\theta_i) = \frac{1}{2\pi}\sin\theta_i \arctanh(\cos\theta_i).
\eeq
We can verify that
\beq
    \left(\frac{\txi^2(\theta_i)}{\sin(2\theta_i)}\right)' =\frac{\arctanh(\cos\theta_i)}{\cos\theta_i}\left(\frac{\arctanh(\cos\theta_i)}{2\cos\theta_i} - 1\right)
\eeq
is indeed monotonic on $[0, \pi/2]$, as well as verify that its critical point value
\beq
    \begin{aligned}
    \xi_c &= \frac{1}{2\pi}\sqrt{\frac{2AK}{\sin(\phi/K)\cos(\phi/K)}}\sin(\phi/K) \arctanh(\cos(\phi/K))\\
    &= \frac{1}{2\pi}\sqrt{2AK\tan(\phi/K)}\arctanh(\cos(\phi/K))
    \end{aligned}
\eeq
is indeed monotonically increasing in $K$ for $K=2s > 2s-2 = 2\phi/\pi$, and so $\xi_c$ is indeed the maximum over the set of \textit{unconstrained triangles} by Lemma 6.2. However, we see that by substituting $\phi$ and $K$, 
\beq
    \begin{aligned}
    \xi_c &= \frac{1}{2\pi}\sqrt{2AK\tan\left(\frac{\pi(s-2)}{2s}\right)}\arctanh\left(\cos\left(\frac{\pi(s-2)}{2s}\right)\right)\\
    &= \frac{1}{\pi}\sqrt{\frac{As}{\tan(\pi/s)}}\arctanh(\sin(\pi/s)) = \bar{\mathbf{r}}_s\sqrt{A}
    \end{aligned}
\eeq
precisely attains the value of the average radius of a regular polygon, and thus must also be the maximum for the constrained set. 
\end{proof}

Noticing that we can also decompose an entire Voronoi tessellation into right triangles, we obtain the next result in the same manner as the previous, by showing the maximum over the unconstrained set is precisely attained to a specific value in the constrained set. 

\begin{Theorem}
The regular hexagon tiling, when admissible, is the global minimum for the Hookean-Voronoi energy. 
\end{Theorem}

\begin{proof}
For a non-degenerate Voronoi tessellation with $N$ sites that lie in $\Omega$, with $|\Omega|=N$ and $M$ vertices, by the Euler characteristic, $M=2N$, since each vertex has 3 edges. We are able to decompose a Voronoi tessellation into $K=6M=12N$ right triangles, with an angle sum constraint of $\sum_{i=1}^K \theta_i = 2\pi M = 4\pi N = \phi$. We can write the sum of the average radii of every Voronoi cell $\bar{r}(\bx)$ in the same way as \eqref{e:barr-triangle-decomp}. As a result, the same verification applies as in the previous proof, and we have that the critical point value for the sum of all the average radii in the system
\beq
    \begin{aligned}
    \xi_c &= \frac{1}{2\pi}\sqrt{\frac{2AK}{\sin(\phi/K)\cos(\phi/K)}}\sin(\phi/K) \arctanh(\cos(\phi/K))\\
    &= \frac{1}{2\pi}\sqrt{2AK\tan(\phi/K)}\arctanh(\cos(\phi/K))
    \end{aligned}
\eeq
is indeed the maximum over the set of \textit{unconstrained triangles} by Lemma 6.2. Substituting, we obtain that
\beq 
    \begin{aligned}
    \xi_c &= \frac{1}{2\pi}\sqrt{24N^2\tan\left(\frac{4\pi N}{12 N}\right)}\arctanh\left(\cos\left(\frac{4\pi N}{12 N}\right)\right)\\
    &\leq \frac{1}{2\pi}N\sqrt{24\tan(\pi/3)} \arctanh(\cos(\pi/3))\\
    &\leq \frac{1}{\pi}N\sqrt{\frac{6}{\tan(\pi/6)}}\arctanh(\sin(\pi/6)) = N\bar{\mathbf{r}}_6.
    \end{aligned}
\eeq

\textcolor{blue}{Still require some algebra to show that $\VEE > 0$}

\end{proof}


%******************************************************************
\subsection{Negative Angles}
\small
Each triangle makes a contribution to the average radius of the tessellation. Since the tessellation has $2N-2<2K$ degrees of freedom, there are many hidden constraints within these parameters that reflect the geometry of the tessellation. We drop these geometric constraints and maximize an extension of the average radius over the collections of $K$ right triangles that satisfy two constraints, one that their total area sums to $N$ and the second that the angles sum to $2\pi N$. Which we maximization over the convex admissible set
 \beq \label{def-Admiss}
 \cA(K):=\left\{Y\,\Bigl |  h_i\in[0,R], \theta_i\in\left[-\frac{\pi}{2},\frac{\pi}{2}\right],\, i=1,\dots, K \right\}.
% & h_i\in[0,R], \theta_i\in\left[-\frac{\pi}{2},0\right], i=K_++1,\ldots, K\Bigr\}
 \eeq
The upper bound $R$ on the hypotenuse of the triangles will be selected sufficiently large, depending only upon $N.$ 

For a non-degenerate Voronoi tessellation, Euler's equation with characteristic zero implies that the tessellation has $3N$ edges. Each tessellation edge abuts two right triangles in each tessellation region, so that a non-degenerate tessellation yields $K=4\cdot3N=12N$ right triangles via the subdivision process. This is the maximum value of $K$. Conversely the constraint on the sum of the angles and their individual range implies that $K\geq 4N$ so that $K\in[4N,12N].$ For $K$ in this range the set $A(K)$ is much larger then the set of right triangles $Y=Y(\bx)$ produced from subdividing the tessellation generated by $\bx$, generically these triangles cannot be reassembled into a Voronoi tessellation of $\Omega_\alpha.$


We apply this Lemma inductively to produce a sharp upper bound on the average radius of a tessellation.
A key point is that the boundary of $\cA(K)$ maps onto $\cA(K-1)$ in the limit that $R\to\infty.$  

\begin{Theorem}
For any $(N,\alpha)$ and any collection of sites, $\bx$, the average radius of the associated tessellation is bounded from above by the average radius of the unit hexagon,
\beq 
\br(\bx)\leq\br_6.
\eeq 
In particular $\VEE(\bx)\geq 0,$ with equality achieved by the hexagonal tessellation when $N\in\cH(\alpha).$ 
\end{Theorem}
\begin{proof}

We fix $N$ and $\alpha$ and consider the set of all right triangle subdivisions of tessellations of $\Omega_\alpha$ by $\bx\in\Omega_\alpha^N.$ Each subdivision forms $K$ right-triangles for some $K\in[4N,12N]$.
To bound the average radius of these tessellations we introduce a convexified family of constrained problems, $\cP(K,\cC)$ for $\cC\in\bR^2.$ These seek to maximize
\beq\label{e:Feq}
F(Y):= \sum_{k=1}^K f(h_k,\theta_k),
\eeq
over $Y\in\cA(K)$, subject to the two constraints,
\beq
\label{e:Ci}
C_i(Y):= \sum_{k=1}^K c_i(h_k,\theta_k) = \cC_i,
%|\Omega_{N,\alpha}|=N,
\eeq
for $i=1,2.$ We make the choices
\begin{align}
    f(h,\theta) &= \frac{1}{2\pi} h \cos\theta \arctanh(\sin \theta)=h \tilde{f}(\theta),
    \label{e:fdef}\\
    %\sin\theta \arctanh(\cos \theta)=h \tilde{f}(\theta), \\
    c_1(h,\theta) &= \frac14 h^2 \sin(2\theta)=h^2\tilde{c}_1(\theta), \label{e:c1def} \\
    c_2(h,\theta) &= \theta.
    \label{e:c2def}
\end{align}
so that if $Y= Y(\bx)$ arises from the partitioning of the tessellation of $\bx$ into right triangles then $\br(\bx)=\frac{1}{N} F(Y(\bx)).$ The constraint values $\cC$ take several forms. The most important is the choice $\cC_1=|\Omega_{\alpha,N}|=N$ and $\cC_2=2\pi N$ for which the constraint on $C_1$ enforces total triangle area $N$ and the constraint on $C_2$ requires that the site angles sum to $2\pi N$. These are the natural values of $\cC$ when $Y=Y(\bx)$ arises as a subdivision of an $N$-site tessellation of $\Omega_{\alpha, N}$.

To apply Lemma\,\ref{l:diagMin} for the choices \eqref{e:fdef}-\eqref{e:c2def} we establish that the resultant function $g$ is one-to-one on $\cA(K)$. We compute that
\beq \label{e:nabla-c} \nabla_y c = 
\begin{pmatrix} 
 2h \tilde{c}_1(\theta)  & 0 \cr
h^2 \tilde{c}_1'(\theta) & 1 
\end{pmatrix},
\eeq
where a prime denotes the derivative of a function of one variable with respect to that variable. The function $g$ takes the form
\beq\label{e:geq} g := 
\begin{pmatrix} \frac{1}{2 h \tilde{c}_1} & 0 \cr
-\frac{h \tilde{c}_1'}{2 \tilde{c}_1} & 1 
\end{pmatrix} 
\begin{pmatrix} \tilde{f} \cr
 h\tilde{f}' 
\end{pmatrix} =
\begin{pmatrix} 
\frac{\tilde{f}}{2 h \tilde{c}_1} \cr
\frac{h}{2} \frac{\tilde{f}'\tilde{c}_1-\tilde{f}\tilde{c}_1'/2}
{\tilde{c}_1} \end{pmatrix} .
%= \begin{pmatrix} \frac{\tilde{f}}{2 h \tilde{c}_1} \cr
%\frac{h\sqrt{|\tilde{c}_1|}}{2} \left(\frac{\tilde{f}}{\sqrt{|\tilde{c}_1|}}\right)'
%\end{pmatrix}.
\eeq
The product  $g_1g_2$ depends only upon $\theta$, so that for Lagrange multipliers $\Lambda=(\lambda_1,\lambda_2)$ the critical point angle $\theta_*$ satisfies 
\beq
\lambda_1\lambda_2=g_1g_2= \frac{1}{8}\left(\frac{\tilde{f}^2}{\tilde{c}_1}\right)'. %=:\tilde{g}(\theta).
\eeq
%\sign(\theta) \frac{\tilde{f}}{4\sqrt{|\tilde{c}_1|}}\left(\frac{\tilde{f}}{\sqrt{|\tilde{c}_1|}}\right)'\!\!(\theta),
The function $\tilde{g}:=\tilde{f}^2/\tilde{c}_1$ has odd parity in $\theta$ about $\theta=0$, and is convex on $(-\pi/2,0)$ and concave on $(0,\pi/2).$ 
In particular $\tilde{g}'$ is even in $\theta$ and concave down. This establishes that $g$ is 1-1 on $[0,R]\times[0,\pi/2]$ and on $[0,R]\times[-\pi/2,0]$. From Lemma\,\ref{l:diagMin} it follows that the critical points of $F$ that are interior to $\cA(K)$ occur at a point of the form $Y_*=(h_*,\pm \theta_*, h_*,\pm \theta_*, \ldots, h_*,\pm\theta_*)\in \bR^{2K}$ for some values $(h_*,\theta_*)\in\bR^2$. For the angle constraint $C_2(Y)=\cC_2$ the negative angle summands precisely cancel an equal number of positive angles yielding 
\beq \label{e:theta*}
\theta_*=\frac{\cC_2}{K-2K_-},
\eeq
where $K_-<K/2$ is the number of negative angles.
%= \frac{\pi}{6},$ 
Similar cancellation in the area constraint $C_1(Y)=\cC_1$ implies that $$h_*=2\sqrt{\frac{\cC_1}{(K-2K_-)\sin(2\theta_*)}}.
%=2\sqrt{\frac{N}{K\sin(4\pi N/K)}}.
$$ 
In particular, defining the  critical values $F_*(K,K_-,\cC):= F(Y_*(K,K_-,\cC))$ we have the suggestive form
\beq\label{e:F*}
%\begin{aligned}
F_* = \sqrt{\cC_1\cC_2} \frac{\cos(\frac{\cC_2}{K_0})\arctanh(\sin(\frac{\cC_2}{K_0}))}
{\pi\sqrt{\frac{\cC_2}{K_0}\sin(2\frac{\cC_2}{K_0})}},
%= \frac{\cos(\frac{2\pi N}{K})\arctanh(\sin(\frac{2\pi N}{K}))} {\pi\sqrt{\frac{N}{K}\sin(\frac{4\pi N}{K})}}.
\eeq
where $K_0=K-2K_-$ is the number of uncanceled triangles. For fixed $\cC,$ the function $F_*$ is monotonically increasing in $K_0$. 
For a given number of right triangles $K$ the interior critical point with the largest value of $F$ occurs for $K_-=0,$ corresponding to all positive angles.

To establish that the constrained maximum does not occur on the boundary of $\cA(K)$ we show that maximum over the boundary can be recast as a problem $\cP$ with modified values for $K$ and $\cC.$ A point $Y\in\partial\cA(K)$ has one or more $i=1, \ldots K$ for which either $\theta_i=\pm \pi/2$ or $h_i=0,R$. If an angle equals $-\pi/2$ then the associated triangle makes no contribution to $F$ and has no area, while contributing $-\pi/2$ to the angle constraint. The maximum of $F$ over $Y$ with one such triangle equals the maximum of $\cP(K-1,\cC_1,\cC_2+\pi/2).$
